Improved No-Regret Algorithms for Stochastic Shortest Path with Linear MDP

We introduce two new no-regret algorithms for the stochastic shortest path (SSP) problem with a linear MDP that significantly improve over the only existing results of (Vial et al., 2021). Our first algorithm is computationally efficient and achieves a regret bound $\widetilde{O}\left(\sqrt{d^3B_{\star}^2T_{\star} K}\right)$, where $d$ is the dimension of the feature space, $B_{\star}$ and $T_{\star}$ are upper bounds of the expected costs and hitting time of the optimal policy respectively, and $K$ is the number of episodes. The same algorithm with a slight modification also achieves logarithmic regret of order $O\left(\frac{d^3B_{\star}^4}{c_{\min}^2\text{gap}_{\min}}\ln^5\frac{dB_{\star} K}{c_{\min}} \right)$, where $\text{gap}_{\min}$ is the minimum sub-optimality gap and $c_{\min}$ is the minimum cost over all state-action pairs. Our result is obtained by developing a simpler and improved analysis for the finite-horizon approximation of (Cohen et al., 2021) with a smaller approximation error, which might be of independent interest. On the other hand, using variance-aware confidence sets in a global optimization problem, our second algorithm is computationally inefficient but achieves the first "horizon-free" regret bound $\widetilde{O}(d^{3.5}B_{\star}\sqrt{K})$ with no polynomial dependency on $T_{\star}$ or $1/c_{\min}$, almost matching the $\Omega(dB_{\star}\sqrt{K})$ lower bound from (Min et al., 2021).

==> app-lb.tex <==
% !TEX root = main.tex

\subsection{\pfref{thm:lb}}
\begin{proof}
	%By Yao's minimax principle, in order to obtain a regret lower bound, it suffices to show that there exists a distribution of SSP instances that forces any deterministic learner to suffer a regret bound of $\Omega(d\B\sqrt{K})$ (or $\lowo{\frac{d\B^2}{\mingap}}$) in expectation.
	Define $\delta=\frac{1}{3}$, $\Delta = \frac{\sqrt{\delta/K}}{8\sqrt{2}}$ and assume $K\geq\frac{d^2}{2\delta}$.
	Consider a family of SSP parameterized by $\rho\in\{-\Delta, \Delta\}^d$ with action set $\calA=\{-1, 1\}^d$.
	For the SSP instance parameterized by $\rho$, it consists of two states $\{s_0, s_1\}$.
	The transition probabilities are as follows:
	\begin{align*}
		&P(s_1|s_0, a) = 1 - \delta - \inner{\rho}{a}, \quad  P(g|s_0, a)=\delta + \inner{\rho}{a},\\
		&P(s_1|s_1, a) = 1 - 1/\B, \quad P(g|s_1, a) = 1/\B,
	\end{align*}
	and the cost function is $c(s, a)=\Ind\{s=s_1\}$.
	The SSP instance above can be represented as a linear SSP of dimension $d+2$ as follows: define $\alpha=\sqrt{\frac{1}{1+\Delta d}}$, $\beta=\sqrt{\frac{\Delta}{1+\Delta d}}$, 
	\begin{align*}
		\phi(s, a) = \begin{cases}
			[\alpha, \beta a^{\top}, 0]^{\top}, & s = s_0\\
			[0, 0, 1]^{\top}, & s = s_1
		\end{cases}\qquad
		\mu(s') = \begin{cases}
			[(1-\delta)/\alpha, -\rho^{\top}/\beta, 1-1/\B]^{\top}, & s'=s_1\\
			[\delta/\alpha, \rho^{\top}/\beta, 1/\B]^{\top}, & s = g
		\end{cases}
	\end{align*}
	and $\thetastar = [0, 0, 1]$.
	Note that it satisfies $c(s, a)=\phi(s, a)^{\top}\thetastar$, $P(s'|s, a)=\phi(s, a)^{\top}\mu(s')$, $\norm{\phi(s, a)}_2\leq 1$, and $\norm{\thetastar}_2\leq 1\leq\sqrt{d+2}$.
	Moreover, for any function $h: \calS_+\rightarrow \fR$, we have:
	\begin{align*}
		\sum_{s'}h(s')\mu(s') = \begin{bmatrix}
			h(s_1)(1-\delta)\sqrt{1+\Delta d} + h(g)\delta\sqrt{1+\Delta d}\\
			(h(g)-h(s_1))\rho\sqrt{(1+\Delta d)/\Delta}\\
			h(s_1)(1-1/\B) + h(g)/\B
		\end{bmatrix}.
	\end{align*} 
	Note that when $K\geq \frac{d^2}{2\delta}$, $\Delta d\leq \frac{\delta}{8}=\frac{1}{24}$, and
	\begin{align*}
		(h(s_1)(1-\delta)\sqrt{1+\Delta d} + h(g)\delta\sqrt{1+\Delta d})^2 &\leq \norm{h}_{\infty}^2(1+\Delta d) \leq \frac{25}{24}\norm{h}_{\infty}^2, \\
		\norm{(h(g)-h(s_1))\rho\sqrt{(1+\Delta d)/\Delta}}_2^2 &\leq 4\norm{h}_{\infty}^2\Delta d(1+\Delta d) \leq \frac{25}{24}\norm{h}_{\infty}^2, \\
		(h(s_1)(1-1/\B) + h(g)/\B)^2 &\leq \norm{h}_{\infty}^2.
	\end{align*}
	Thus, we have $\norm{\sum_{s'}h(s')\mu(s')}_2\leq \norm{h}_{\infty}\sqrt{d+2}$ by $d\geq 2$.
	The regret is bounded as follows: let $a_k$ denote the first action taken by the learner in episode $k$.
	Then for any $\rho\in\{-\Delta, \Delta\}^d$, the expected cost of taking action $a$ as the first action is $C_{\rho}(a)=\B(1-\delta-\inner{\rho}{a})$.
	\begin{align*}
		\E_{\rho}[R_K] &= \sumk\E_{\rho}\sbr{C_{\rho}(a_k) - \min_aC_{\rho}(a)} \\
		&= \B\sumk\E_{\rho}\sbr{\max_a\inner{\rho}{a} - \inner{\rho}{a_k}} \\
		&= 2\B\Delta\sumk\E_{\rho}\sbr{ \sum_{j=1}^d \Ind\{\sgn(\rho_j) \neq \sgn(a_{k,j})\} } \\
		&= 2\B\Delta\sum_{j=1}^d\E_{\rho}[N_j(\rho)],
	\end{align*}
	where we define $N_j(\rho)=\sumk \Ind\{\sgn(\rho_j) \neq \sgn(a_{k,j})\}$, and $\E_{\rho}$ is the expectation w.r.t the SSP instance parameterized by $\rho$.
	Let $\rho^j$ denote the vector that differs from $\rho$ at its $j$-th coordinate only.
	Then, we have $N_j(\rho^j) + N_j(\rho) = K$, and for a fixed $j$,
	\begin{align*}
		2\sum_{\rho}\E_{\rho}\sbr{R_K} &= \sum_{\rho}\rbr{\E_{\rho}\sbr{R_K} + \E_{\rho^j}\sbr{R_K}}\\
		&= 2\B\Delta\sum_{\rho}\sum_{j=1}^d\rbr{ K + \E_{\rho}[N_j(\rho)] - E_{\rho^j}[N_j(\rho)] }\\
		&\geq 2\B\Delta\sum_{\rho}\sum_{j=1}^d\rbr{ K - K\sqrt{2\KL(P_{\rho}, P_{\rho^j})} },
	\end{align*}
	where $P_{\rho}$ is the joint probability of $K$ trajectories induced by the interactions between the learner and the SSP parameterized by $\rho$, and in the last inequality we apply Pinsker's inequality to obtain:
	\begin{align*}
		\abr{\E_{\rho}[N_j(\rho)] - \E_{\rho^j}[N_j(\rho)]} \leq K\norm{P_{\rho}-P_{\rho^j}}_1 \leq K\sqrt{2\KL(P_{\rho}, P_{\rho^j})}. %&\leq \sum_{\tau_{1:K}}|P_{\rho}(\tau_{1:K}) - P_{\rho^j}(\tau_{1:K})|N_j(\rho)(\tau_{1:K})\\
		%&\leq K\sum_{\tau_{1:K}}|P_{\rho}(\tau_{1:K}) - P_{\rho^j}(\tau_{1:K})|\\
		%&\leq K\sqrt{2\KL(P_{\rho}, P_{\rho^j})}, \tag{Pinsker's inequality}
	\end{align*}
	By the divergence decomposition lemma (see e.g.~\citep[Lemma~15.1]{lattimore2020bandit}) and the fact that the cost is known while the transition is unknown to the learner, we further have
	\begin{align*}
		\KL(P_{\rho}, P_{\rho^j}) &= \sumk \E_{\rho}\sbr{\KL\rbr{\bernoulli(\delta + \inner{a_k}{\rho}), \bernoulli(\delta+\inner{a_k}{\rho^j})}} \\ 
		&= \sumk \E_{\rho}\sbr{ \frac{2\inner{a_k}{\rho-\rho^j}^2}{\delta + \inner{a_k}{\rho}} } \leq \frac{16K\Delta^2}{\delta},\tag{$d\Delta\leq\delta/2$}
		%\KL(P_{\rho}, P_{\rho^j}) &= \sum_{\tau_{1:K}}P_{\rho}(\tau_{1:K})\ln\frac{P_{\rho}(\tau_{1:K})}{P_{\rho^j}(\tau_{1:K})} = \sumk\sum_{\tau_{1:k}}P_{\rho}(\tau_{1:k})\ln\frac{P_{\rho}(\tau_k|\tau_{1:k-1})}{P_{\rho^j}(\tau_k|\tau_{1:k-1})}\\
		%&= \sumk\sum_{\tau_{1:k-1}}P_{\rho}(\tau_{1:k-1})\sum_{s_{k,2}}P(s_{k,2}|\tau_{1:k-1})\ln\frac{P_{\rho}(s_{k,2}|\tau_{1:k-1})}{P_{\rho^j}(s_{k,2}|\tau_{1:k-1})}\\
		%&= \sumk\sum_{\tau_{1:k-1}}P_{\rho}(\tau_{1:k-1})\KL(\bernoulli(\delta + \inner{a_k}{\rho}), \bernoulli(\delta+\inner{a_k}{\rho^j}))\\
		%&\leq \sumk \E_{\rho, \tau_{1:k-1}}\sbr{ \frac{2\inner{a_k}{\rho-\rho^j}^2}{\delta + \inner{a_k}{\rho}} } \leq \frac{16K\Delta^2}{\delta}. \tag{$d\Delta\leq\delta/2$}
	\end{align*}	
%	By the chain rule of relative entropy, $\KL(P_{\rho}, P_{\rho^j})$ can be further decomposed as (note that we only need to consider the state sequence since the cost is known):
%	\begin{align*}
%		\KL(P_{\rho}, P_{\rho^j}) &= \sum_{\tau_{1:K}}P_{\rho}(\tau_{1:K})\ln\frac{P_{\rho}(\tau_{1:K})}{P_{\rho^j}(\tau_{1:K})} = \sumk\sum_{\tau_{1:k}}P_{\rho}(\tau_{1:k})\ln\frac{P_{\rho}(\tau_k|\tau_{1:k-1})}{P_{\rho^j}(\tau_k|\tau_{1:k-1})}\\
%		&= \sumk\sum_{\tau_{1:k-1}}P_{\rho}(\tau_{1:k-1})\sum_{s_{k,2}}P(s_{k,2}|\tau_{1:k-1})\ln\frac{P_{\rho}(s_{k,2}|\tau_{1:k-1})}{P_{\rho^j}(s_{k,2}|\tau_{1:k-1})}\\
%		&= \sumk\sum_{\tau_{1:k-1}}P_{\rho}(\tau_{1:k-1})\KL(\bernoulli(\delta + \inner{a_k}{\rho}), \bernoulli(\delta+\inner{a_k}{\rho^j}))\\
%		&\leq \sumk \E_{\rho, \tau_{1:k-1}}\sbr{ \frac{2\inner{a_k}{\rho-\rho^j}^2}{\delta + \inner{a_k}{\rho}} } \leq \frac{16K\Delta^2}{\delta}. \tag{$d\Delta\leq\delta/2$}
%	\end{align*}
	where in the second last inequality we apply $\KL(\bernoulli(a), \bernoulli(b))\leq 2(a-b)^2/a$ when $a\leq 1/2, a+b\leq 1$, which is true when $\delta\leq 1/3$, $d\Delta\leq\delta/2$.
	Substituting these back, we get:
	\begin{align}
		2\sum_{\rho}\E_{\rho}[R_K] \geq 2\B\Delta\sum_{\rho}\sum_{j=1}^d\rbr{K - K\sqrt{32K\Delta^2/\delta}} = \lowO{\sum_{\rho} d\B\sqrt{\delta K}}. \label{eq:lb}
	\end{align}
	%Selecting $\rhostar$ which maximizes $\E_{\rho}[R_K]$, we get: $\E_{\rhostar}[R_K]= \lowo{d\B\sqrt{K}}$.
	%For the gap-dependent logarithmic lower bound, note that $\gap(s_1, a)=0$ for all $a$.
	Now note that $\gap(s_1, a)=0$ for all $a$.
	Define $\astar=\argmax_a\inner{\rho}{a}$.
	Then for any $a\neq \astar$,
	\begin{align*}
		\optQ(s_0, a) - \optV(s_0) = (1-\delta-\inner{\rho}{a})\B - (1-\delta-\inner{\rho}{\astar})\B = \B\inner{\rho}{\astar-a} \geq 2\B\Delta.
	\end{align*}
	Thus, $\mingap = 2\B\Delta$.
	By $\sqrt{K}=\frac{\sqrt{\delta}}{8\sqrt{2}\Delta}$ and \pref{eq:lb}, we get:
	\begin{align*}
		\sum_{\rho}\E_{\rho}[R_K] = \lowO{\sum_{\rho}\B d\sqrt{\delta K}} = \lowO{ \sum_{\rho}\frac{d\B\delta}{\Delta} } = \lowO{\sum_{\rho}\frac{d\B^2}{\mingap} }.
	\end{align*}
	Selecting $\rhostar$ which maximizes $\E_{\rho}[R_K]$, we get: $\E_{\rhostar}[R_K]= \lowO{\frac{d\B^2}{\mingap}}$.
\end{proof}

%\begin{remark}
%	Similar to \cite{zhou2021nearly}, we can prove the same lower bound for a related MDP class called linear mixture SSP, which assumes finite number of states and actions, a known cost function $c$, a known feature map $\phi:\SA\times\calS^+\rightarrow \fR^d$, and an unknown vector $\thetastar\in\fR^d$ with $\norm{\thetastar}_2\leq B$ for some constant $B$, such that:
%\begin{itemize}
%	\item for any $(s, a), s'\in\SA\times\calS^+$, we have $P_{s, a}(s')=\phi(s'|s, a)^{\top}\thetastar$;
%	\item for any bounded function $F:\calS\rightarrow [0, 1]$, we have $\norm{\phi_F(s, a)}_2\leq 1$, where $\phi_F(s, a)=\sum_{s'}\phi(s'|s, a)F(s')\in\fR^d$.
%\end{itemize}
%	To prove the same lower bound for linear mixture SSP, it suffices to show that the class of SSP instances above are also a class of linear mixture SSP instances.
%	The parameterization is as follows: define $\thetastar = [1/\alpha, \rho^{\top}/\beta, 1/\gamma\B]^{\top}$, and
%	\begin{align*}
%		\phi(s'|s, a) = \begin{cases}
%			[\alpha(1-\delta), -\beta a^{\top}, 0]^{\top},& s = s_0, s' = s_1\\
%			[\alpha\delta, \beta a^{\top}, 0]^{\top},& s = s_0, s' = g \\
%			[\alpha, 0, -\gamma]^{\top},& s = s_1, s' = s_1 \\
%			[0, 0, \gamma]^{\top},& s = s_1, s' = g
%		\end{cases}
%	\end{align*}
%	where $\alpha = \sqrt{\frac{1}{1+\Delta d + 1/\B}}$, $\beta=\sqrt{\frac{\Delta}{1+\Delta d + 1/\B}}$, and $\gamma = \sqrt{\frac{1/\B}{1 + \Delta d + 1/\B}}$.
%	It is straightforward to verify that $P(s'|s, a)=\phi(s'|s, a)^{\top}\thetastar$.
%	Note that $\norm{\thetastar}_2^2=(1 + \Delta d + 1/\B)^2\leq (2+\delta/8)^2\leq 9$.
%	Moreover, for any $F:\calS^+\rightarrow [0, 1]$:
%	\begin{align*}
%		\phi_F(s_0, a) &= [F(s_1)\alpha(1-\delta) + F(g)\alpha\delta, \beta(F(g)-F(s_1))a^{\top}, 0]^{\top},\\
%		\phi_F(s_1, a) &= [\alpha F(s_1), 0, \gamma(F(g)-F(s_1))]^{\top},
%	\end{align*}
%	which implies that $\norm{\phi_F(s_0, a)}_2\leq 1$ and $\norm{\phi_F(s_1, a)}_2\leq 1$.
%	Thus, it is a linear mixture SSP with $B=9$.
%\end{remark}

